Irregularly Tabulated MLP for Fast Point Feature Embedding

Aiming at drastic speedup for point-feature embeddings at test time, we propose a new framework that uses a pair of multi-layer perceptrons (MLP) and a lookup table (LUT) to transform point-coordinate inputs into high-dimensional features. When compared with PointNet's feature embedding part realized by MLP that requires millions of dot products, the proposed framework at test time requires no such layers of matrix-vector products but requires only looking up the nearest entities from the tabulated MLP followed by interpolation, defined over discrete inputs on a 3D lattice that is substantially arranged irregularly. We call this framework LUTI-MLP: LUT Interpolation ML that provides a way to train end-to-end irregularly tabulated MLP coupled to a LUT in a specific manner without the need for any approximation at test time. LUTI-MLP also provides significant speedup for Jacobian computation of the embedding function wrt global pose coordinate on Lie algebra $\mathfrak{se}(3)$ at test time, which could be used for point-set registration problems. After extensive evaluation using the ModelNet40, we confirmed that the LUTI-MLP even with a small (e.g., $4^3$) lattice yields performance comparable to that of the MLP while achieving significant speedup: $100\times$ for the embedding, $12\times$ for the approximate Jacobian, and $860\times$ for the canonical Jacobian.

==> fig/network_irr.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width=1\columnwidth]{fig/network_irr_.pdf}
\end{center}
\caption{
\label{fig:network_irr}
\textbf{LUTI-MLP using irregular lattice.}
PointNet by using our LUTI-MLP at test time.
At test time, 8 embedding basis function $\mathbf{\bar{z}}_i^{(j)}$ pre-computed from 8 discrete neighborhood points on the input space lattice $\mathbb{D}^3$ is linearly interpolated (trilinear interpolation) to compute the embedding vector for input $\mathbf{p}_i=[x,y,z]$ in $\mathbb{R}^3$, 
as  $\mathbf{z}_{i}=\sum w_i^{(j)}\mathbf{\bar{z}}_i^{(j)}$.
Only difference with LUTI with regular lattice is it use two LUT and taking point-wise $\min$ operation.
This operation effectively shift lattice location thus utilize more inputs points.
}
\end{figure*}



==> table/modelnet_ft.tex <==
\begin{table}[t]
\caption{
\label{table:modelnet_ft}
\textbf{Results with T-Net (FT)  on ModelNet40 \cite{wu20153d} classification task.}
For all the results, T-Net (FT) is used in combination with T-Net (IT).
We compare the results from PointNet with MLP and one with our LUTI-MLP.
MLP IT+FT represents the original PointNet with IT+FT (with orthogonal regularization).
IT+FT (mod) represents modified version of T-Net shown in \Fig \ref{fig:tnet}.
Results using different discretization $D$ are shown for LUTI-MLP, and the result using MLP are shown in column $\inf$.
Our E2E trained PointNet with LUT-MLP achieves comparable results as original architecture while achieving significant speed-up.
}

\begin{center}
\begin{tabular}{cc|cccccc}
\multicolumn{2}{c}{  } & \multicolumn{6}{c}{discretization $D$} \\ \hdashline
\multicolumn{2}{c}{ architecture } & $\inf$ & 64 & 32 & 16 & 8 & 4 \\ \hline
MLP & IT+FT & 86.47\% & - & - & - & - & - \\ \hdashline
MLP & IT+FT(mod) & 85.74\% & - & - & - & - & - \\ \hdashline
LUT-MLP Approx. & IT+FT(mod) & - & 85.45\% & 84.28\% & 80.92\% & 42.63\% & 11.18\% \\
LUTI-MLP Approx. & IT+FT(mod) & - & 84.52\% & 80.71\% & 54.78\% & 19.08\% & 9.89\% \\ \hdashline
LUTI-MLP E2E & IT+FT(mod) & - & 85.37\% & 85.58\% & 84.77\% & 86.02\% & 84.77\% \\
\end{tabular}

\end{center}
\end{table}
